ColoRadar: The Direct 3D Millimeter Wave Radar Dataset

Millimeter wave radar is becoming increasingly popular as a sensing modality for robotic mapping and state estimation. However, there are very few publicly available datasets that include dense, high-resolution millimeter wave radar scans and there are none focused on 3D odometry and mapping. In this paper we present a solution to that problem. The ColoRadar dataset includes 3 different forms of dense, high-resolution radar data from 2 FMCW radar sensors as well as 3D lidar, IMU, and highly accurate groundtruth for the sensor rig's pose over approximately 2 hours of data collection in highly diverse 3D environments.

==> tikz/physical_array.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
width=4.5cm,
height=3.0cm,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black}
]
\addplot [only marks, mark=*, draw=blue, fill=blue, colormap/viridis]
table{%
x                      y
0 0
0.5 0
1 0
1.5 0
};
\addplot [only marks, mark=*, draw=red, fill=red, colormap/viridis]
table{%
x                      y
2 0
4 0
};
\end{axis}

\end{tikzpicture}


==> tikz/virtual_array.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\begin{axis}[
width=4.5cm,
height=3.0cm,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black}
]
\addplot [only marks, mark=*, draw=green!50!black, fill=green!50!black, colormap/viridis]
table{%
x                      y
1 0
1.25 0
1.5 0
1.75 0
2 0
2.25 0
2.5 0
2.75 0
};
\end{axis}

\end{tikzpicture}

